Anomaly Detection with Joint Representation Learning of Content and Connection

Social media sites are becoming a key factor in politics. These platforms are easy to manipulate for the purpose of distorting information space to confuse and distract voters. Past works to identify disruptive patterns are mostly focused on analyzing the content of tweets. In this study, we jointly embed the information from both user posted content as well as a user's follower network, to detect groups of densely connected users in an unsupervised fashion. We then investigate these dense sub-blocks of users to flag anomalous behavior. In our experiments, we study the tweets related to the upcoming 2019 Canadian Elections, and observe a set of densely-connected users engaging in local politics in different provinces, and exhibiting troll-like behavior.

==> cmds.tex <==
% COMMANDS AND HOTKEYS 
%\mathbb commands.
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\J}{\mathbb{J}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\usepackage{bbm}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\0}{\mathbbm{0}}

%\mathcal commands.
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\Cs}{\mathcal{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\K}{\mathcal{K}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\ps}{\mathcal{P}}
\newcommand{\Rc}{\mathcal{R}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\hbt}{\frac{\hbar}{2}}

%text shortcuts.
\newcommand{\dne}{\text{ DNE}}
\newcommand{\und}{\text{ undefined}}
\newcommand{\ad}{\text{ and }}
\newcommand{\fs}{\text{ for some }}
\newcommand{\we}{\text{ where }}
\newcommand{\wee}{\text{ where:}}
\newcommand{\st}{\text{ such that }}
\newcommand{\stt}{\text{ such that:}}
\newcommand{\wh}{\text{ we have }}
\newcommand{\wht}{\text{ we have that }}
\newcommand{\wi}{\text{ with }}
\newcommand{\el}{Euler-Lagrange Equation }
\newcommand{\eln}{Euler-Lagrange Equation}
\newcommand{\els}{Euler-Lagrange Equations }
\newcommand{\elsn}{Euler-Lagrange Equations}
\newcommand{\he}{Hamilton Equation }
\newcommand{\hen}{Hamilton Equation}
\newcommand{\hes}{Hamilton Equations }
\newcommand{\hesn}{Hamilton Equations}
\newcommand{\hje}{Hamilton-Jacobi Equation }
\newcommand{\hjen}{Hamilton-Jacobi Equation}
\newcommand{\sa}{$\sigma$-algebra }
\newcommand{\san}{$\sigma$-algebra}

%math single character shortcuts.
\newcommand{\fa}{\forall}
\newcommand{\eq}{\exists}
\newcommand{\imp}{\implies}
\newcommand{\dnimp}{\centernot\implies}
\newcommand{\cd}{\cdot}
\newcommand{\ceq}{\coloneqq} % :=
\newcommand{\sbs}{\subseteq}
\newcommand{\sps}{\supseteq}
\newcommand{\nsbs}{\not\subseteq}
\newcommand{\nsps}{\not\supseteq}
\newcommand{\nin}{\notin}
\newcommand{\sqsbs}{\sqsubseteq} % square subseteq

%math shortcut commands.
\newcommand{\Bp}{\B^\ast}
\newcommand{\f}{f^{-1}}
\newcommand{\e}{\varepsilon}
\newcommand{\de}{\delta}
\newcommand{\es}{\emptyset}
% \newcommand{\lp}{\ell^p}
\newcommand{\sm}{\setminus}
\newcommand{\p}{\partial}
\newcommand{\pr}{\, '}
% \newcommand{\indep}{\ensuremath{\! \! \perp \! \! \! \perp \!}}
\newcommand{\vf}{\vec{F}}
\newcommand{\vtau}{\vec{\tau}}
\newcommand{\vnab}{\vec{\nabla}} %vector gradient
\newcommand{\dotp}{\dot{\mathcal{P}}}
\newcommand{\dotq}{\dot{\mathcal{Q}}}
% \newcommand{\norm}{\| \circ \|}
\newcommand{\Co}{ \Cs \left( 0,1 \right) }
\newcommand{\Ca}{ \Cs \left( a,b \right) }
\newcommand{\FF}{ \{ F_\alpha \}_{\alpha \in I}}
\newcommand{\GG}{ \{ G_\alpha \}_{\alpha \in I}}
\newcommand{\HH}{ \{ H_\alpha \}_{\alpha \in I}}
\newcommand{\KK}{ \{ K_\alpha \}_{\alpha \in I}}
\newcommand{\Ro}{ \mathcal{R} \left( \left[ 0,1 \right] \right) }
\newcommand{\Ra}{ \mathcal{R} \left( \left[ a,b \right] \right) }
\newcommand{\UU}{ \{ U_\alpha \}_{\alpha \in I}}
\newcommand{\Vp}{\V^\ast}
\newcommand{\QC}{\R \sm \Q}
\newcommand{\Sigmast}{\Sigma^\ast}
\newcommand{\deast}{\de^\ast}
\newcommand{\De}{\Delta}
\newcommand{\Deast}{\De^{\hspace{-0.15 em}\ast}}
\newcommand{\Fhat}{\hat{F}}

% paired delimiters: 
\DeclarePairedDelimiter\expect{\E\big[}{\big]} % expectation
\DeclarePairedDelimiter\vari{\mathbb{V}\big[}{\big]}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2} %inner product
\DeclarePairedDelimiter\absd{\lvert}{\rvert} % absolute val
\DeclarePairedDelimiter\normd{\lVert}{\rVert} % norm
\newcommand{\expectauto}[1]{\E\left[#1\right]} % expectation: auto adjusting
\newcommand{\cov}[1]{\operatorname{Cov}\left[#1\right]}
\newcommand{\corr}[1]{\operatorname{Corr}\left[#1\right]}

% automatic \left\right brackets 
\newcommand{\bpar}[1]{\left(#1\right)}
\newcommand{\bbr}[1]{\left[#1\right]}
\newcommand{\bcurly}[1]{\left\{#1\right\}}

% sums 
\newcommand{\sumlimin}{\sum_{i=1}^n}
\newcommand{\sumlimkn}{\sum_{k=1}^n}
\newcommand{\sumlimizn}{\sum_{i=0}^n}
\newcommand{\sumlimkzn}{\sum_{k=0}^n}
\newcommand{\sumlimyzinf}{\sum_{y=0}^\infty}
\newcommand{\sumlimyoinf}{\sum_{y=1}^\infty}
\newcommand{\sumlimiinf}{\sum_{i=-\infty}^\infty}
\newcommand{\intinfinf}{\int_{-\infty}^\infty }
\newcommand{\sumlimiN}{\sum_{i=1}^N}

%command shortcuts.
\newcommand{\ds}{\displaystyle}
\newcommand{\no}{\noindent}
\newcommand{\vs}{\vspace*}
\newcommand{\hs}{\hspace}
\newcommand{\bs}{\baselineskip}

%Griffiths curly r (vector).
\usepackage{calligra}
    \DeclareMathAlphabet{\mathcalligra}{T1}{calligra}{m}{n}
    \DeclareFontShape{T1}{calligra}{m}{n}{<->s*[2.2]callig15}{}
    \newcommand{\rsep}{\ensuremath{\mathcalligra{r \hs{0.15cm}}}}

% probability: P(A | B) (given)
\newcommand\given[1][]{\:#1\vert\:}
